Ms-senet: Enhancing Speech Emotion Recognition Through Multi-scale Feature Fusion With Squeeze-and-excitation Blocks

Speech Emotion Recognition (SER) has become a growing focus of research in human-computer interaction. Spatiotemporal features play a crucial role in SER, yet current research lacks comprehensive spatiotemporal feature learning. This paper focuses on addressing this gap by proposing a novel approach. In this paper, we employ Convolutional Neural Network (CNN) with varying kernel sizes for spatial and temporal feature extraction. Additionally, we introduce Squeeze-and-Excitation (SE) modules to capture and fuse multi-scale features, facilitating effective information fusion for improved emotion recognition and a deeper understanding of the temporal evolution of speech emotion. Moreover, we employ skip connections and Spatial Dropout (SD) layers to prevent overfitting and increase the model's depth. Our method outperforms the previous state-of-the-art method, achieving an average UAR and WAR improvement of 1.62% and 1.32%, respectively, across six benchmark SER datasets. Further experiments demonstrated that our method can fully extract spatiotemporal features in low-resource conditions.

==> Table/Ablation1.tex <==

\begin{table*}[]
\renewcommand{\arraystretch}{1.0}
% \small
\centering
\caption{The average performance of ablation studies and \methodname under 10-fold CV on all six corpora. The `w/o' means removing the component from \methodname.}
\begin{tabular*}{1\linewidth}{@{\extracolsep{\fill}}rcccccc}
\toprule[1.5pt]
\textbf{Dataset} & \textbf{Metrics} & \textbf{TCN} & \textbf{w/o Bi} & \textbf{w/o MS} & \textbf{w/o DF} & \textbf{\methodname} \\ \midrule
\textbf{CASIA} & \tabincell{\boldmath $\mathrm{UAR}$\\\boldmath $\mathrm{WAR}$} & \tabincell{86.92\\86.92}   & \tabincell{91.33\\91.33}      & \tabincell{90.50\\90.50}     & \tabincell{91.83\\91.83}        & \tabincell{\textbf{94.67}\\\textbf{94.67}} \\\midrule
\textbf{EMODB} & \tabincell{\boldmath $\mathrm{UAR}$\\\boldmath $\mathrm{WAR}$}    & \tabincell{89.68\\90.09}    & \tabincell{90.96\\91.59}      & \tabincell{91.80\\92.52}     & \tabincell{91.46\\92.34}        & \tabincell{\textbf{95.17}\\\textbf{95.70}} \\\midrule
\textbf{EMOVO} & \tabincell{\boldmath $\mathrm{UAR}$\\\boldmath $\mathrm{WAR}$}    & \tabincell{82.14\\82.14}   & \tabincell{86.73\\86.73}      & \tabincell{87.24\\87.24}     & \tabincell{86.56\\86.56}        & \tabincell{\textbf{92.00}\\\textbf{92.00}} \\\midrule
\textbf{IEMOCAP} & \tabincell{\boldmath $\mathrm{UAR}$\\\boldmath $\mathrm{WAR}$}  & \tabincell{61.97\\59.84}    & \tabincell{71.07\\70.22}      & \tabincell{70.68\\70.04}     & \tabincell{70.82\\69.82}        & \tabincell{\textbf{72.50}\\\textbf{71.65}} \\\midrule
\textbf{RAVDESS} & \tabincell{\boldmath $\mathrm{UAR}$\\\boldmath $\mathrm{WAR}$}  & \tabincell{83.20\\83.75}    & \tabincell{88.48\\88.68}      & \tabincell{89.97\\90.21}     & \tabincell{87.50\\87.99}        & \tabincell{\textbf{91.93}\\ \textbf{92.08}} \\\midrule
\textbf{SAVEE} & \tabincell{\boldmath $\mathrm{UAR}$\\\boldmath $\mathrm{WAR}$}    & \tabincell{78.81\\80.63}    & \tabincell{80.95\\83.33}      & \tabincell{82.50\\84.38}     & \tabincell{80.95\\82.92}        & \tabincell{\textbf{86.31}\\\textbf{87.71}}\\
\bottomrule[1.5pt]


\end{tabular*}
\label{tab:ablation}
\end{table*}

==> Table/Generalizability.tex <==
\begin{table}[]
\renewcommand{\arraystretch}{1.0}
\small
\centering
\caption{UAR and WAR on the cross-corpus SER task with different methods. All values are the average $\pm$ std of 10 runs, each of which consists of 20 cross-corpus cases.}
\begin{tabular*}{1\linewidth}{@{\extracolsep{\fill}}cccc}
\toprule[1.5pt]
\addline{\textbf{Method}}  & \textbf{TCN}         & \textbf{CAAM}~\cite{CPAC_IJCAI}                        & \textbf{\methodname}\\\midrule
\addline{\textbf{\tabincell{\boldmath $\mathrm{UAR}_\mathrm{avg} \pm \mathrm{std}$\\\boldmath $\mathrm{WAR}_\mathrm{avg} \pm \mathrm{std}$}}} & \tabincell{24.47 $\pm$ 0.38\\24.39 $\pm$ 0.42}                     & \tabincell{32.37 $\pm$ 0.27\\33.65 $\pm$ 0.41}                         & \textbf{\tabincell{34.49 $\pm$ 0.43\\35.66 $\pm$ 0.32}}\\
\bottomrule[1.5pt]
\end{tabular*}
\label{tab:generalization}
\end{table}




